Revenue Maximization of Airbnb Marketplace using Search Results

Correctly pricing products or services in an online marketplace presents a challenging problem and one of the critical factors for the success of the business. When users are looking to buy an item they typically search for it. Query relevance models are used at this stage to retrieve and rank the items on the search page from most relevant to least relevant. The presented items are naturally "competing" against each other for user purchases. We provide a practical two-stage model to price this set of retrieved items for which distributions of their values are learned. The initial output of the pricing strategy is a price vector for the top displayed items in one search event. We later aggregate these results over searches to provide the supplier with the optimal price for each item. We applied our solution to large-scale search data obtained from Airbnb Experiences marketplace. Offline evaluation results show that our strategy improves upon baseline pricing strategies on key metrics by at least +20% in terms of booking regret and +55% in terms of revenue potential.

==> HomePricing.tex <==

\pv{Puya, We need to see if there are other apporaches to compare with.}


In this section, we adapted the customized regression model (CRM) proposed in \cite{ye2018customized} for Airbnb Home Dynamic Pricing to Airbnb Experiences. We implemented this state-of-art method from scratch and made several adaptations so as to make it work for Experiences data.

\subsection{Related Work and Adaptation}
The CRM model consists of two components: a booking probability model that predicts whether an available future night of a specific listing will be booked as of the day when making prediction, plus a second strategy model which maps booking probability to price suggestion. Specifically, the price suggestion is centered at a pivot price, and is decreased or increased by a magnitude which is a non-linear function of booking probability. The non-linear function contains parameters learned by minimizing a customized loss function. 

\subsubsection{Booking probability Model}
In CRM, the booking probability model (BPM) predicts, for a given listing at a specific date $ds$, the cumulative probability $P_r$ that a future $ds\_night$ will be booked from $ds$ at different prices. The model uses features including lead time, supply and demand, and listing features. We replace this booking probability model with an occupancy rate model, which predicts for each instance that starts in the next $28$ days, the probability that the occupancy rate is in a range $(a, b]$ when the price is set at some pivot price, namely,
\begin{equation}
    Pr(occrate \in (a,b] | X_ds ,ds_{night}, ds_{night hour}, P_{pivot}),
\end{equation}
where $X_ds$ is the features of an experience instance. This model predicts for the next $28$ days, the occupancy rate for each experience instance, and the probability of booking is a special case when $a=0, b=\infty$. 
{\color{red}{Hi Puya, could you check about this occupancy rate model?}}

Due to the challenges in demand estimation, instead of directly maximizing the revenue using the booking probability Model, a better choice is to construct a strategy model which compute optimal price based on some targeted metrics and use the estimated demand at the pivot price $P_{pivot}$ as input to this model. Then the price suggestion is obtained via the following non-linear transformation of $P_r$,

\begin{equation}
  P_{sugg} = P\cdot V = P_{pivot} \cdot  \left\{
                \begin{array}{ll}
                  1 + \theta_1(P_r(P_{pivot})^{\phi_H^{-P_r D}}-\theta_2), \ \ if \ D \geq 0 \\
                  1 + \theta_1(P_r(P_{pivot})^{\phi_L^{-(1-P_r)D}}-\theta_2), \ \ if \ D \geq 0,                  
                \end{array}
              \right.
\end{equation}
where $P_{pivot}$ could be the most representative calendar price set by the host. $P_r(P_{pivot})$ is the booking probability estimated at price $P_{pivot}$ from the first model.
$\theta_1$ and $\theta_2$ are parameters learned in the strategy model. $D$ is a normalized demand score, and in our experiment, we set it to be the ratio of bookings over all available instances in the last 30 days, and normalize it on $[-1,1]$.


\subsubsection{Strategy Model}

The second strategy layer takes the (price, probability) as a input, and learn the optimal price so as to minimize the loss of making 'bad' price suggestions. They define the lower bound and upper bound of the optimal price range as \begin{equation}
\begin{aligned}
    L(P_i, y_i) &= y_i \cdot P_i + (1-y_i)\cdot c_1 P_i \\
    U(P_i, y_i) & = (1-y_i) \cdot P_i + y_i \cdot c_2 P_i,
\end{aligned}
\end{equation}
where $c_1$ and $c_2$ are two hyper-parameters to tune for the best performance in terms of the defined metrics. The objective function is defined as 
\begin{equation}
    \mathcal{L} = \argmin_{\theta} \sum_{i=1}^N(L(P_i, y_i) - f_{\theta}(x_i))^{+} + (f_{\theta}(x_i) - U(P_i, y_i))^{+},
\end{equation}
where $f_{\theta}$ is assumed to be of an asymmetric exponential form.

The original CRM model was trained on listing level of homes. However, for experiences, due to less price dynamics, the learning of $\theta_1$ and $\theta_2$ at the instance level is not ideal. We aggregate experiences at market-category level during the training.

\subsection{Price recommendation}
After model training, we learn $\theta_1$ and $\theta_2$ at a market-category level, and then make price suggestion at an instance level for instances in the testing set, using the predicted booking probability from our occupancy rate model. We average price suggestion for each instance in the testing set to get aggregated price suggestion for each experience.


\begin{comment}
\begin{itemize}
    \item features used to train the model: {\color{red}{Same features that are used in the occupancy model built by Puya, plus the listing price for each instance.}}
    \item the objective of learning is to predict whether an available future night of a specific listing will be booked as of the day we make this prediction. Therefore during the model training, for each date (ds), the model predicts future available listing nights, and compute the loss. 
\end{itemize}
\end{comment}

==> applications.tex <==
%!TEX root = paper.tex
%
\begin{comment}
\begin{itemize}
    \item We try to build a lookup table or somehow some structure that has some info on what should be the price vector (sort of saving it for top cases);
    \item  we can try to see what would be the best item to add for maximal revenue. Given a set of items we select n of them, and we run your algorithm, we see the revenue, and we choose which item to add, that maximize the revenue;
    \item we look at the data of top10 results coming from search, we find the price vector, and we it many times. We than average over all the prices found and we say this should be the price for this item (given the context that the item is usually appearing it).
if we can figure out a way to have the price vector in less than 50ms, than we can do also online experiments.
\end{itemize}
\end{comment}


